Evidential Active Recognition: Intelligent and Prudent Open-World Embodied Perception

Active recognition enables robots to intelligently explore novel observations, thereby acquiring more information while circumventing undesired viewing conditions. Recent approaches favor learning policies from simulated or collected data, wherein appropriate actions are more frequently selected when the recognition is accurate. However, most recognition modules are developed under the closed-world assumption, which makes them ill-equipped to handle unexpected inputs, such as the absence of the target object in the current observation. To address this issue, we propose treating active recognition as a sequential evidence-gathering process, providing by-step uncertainty quantification and reliable prediction under the evidence combination theory. Additionally, the reward function developed in this paper effectively characterizes the merit of actions when operating in open-world environments. To evaluate the performance, we collect a dataset from an indoor simulator, encompassing various recognition challenges such as distance, occlusion levels, and visibility. Through a series of experiments on recognition and robustness analysis, we demonstrate the necessity of introducing uncertainties to active recognition and the superior performance of the proposed method.

==> deprecated.tex <==
\begin{table*}[t]
\centering
\footnotesize
\caption{Recognition success rate on the proposed dataset. 
% The results are reported based on predictions made at the final step. 
{\texttt{Random}} and {\texttt{Fixation}} two heuristic policies, while {\texttt{G.T. tracking}} implies the direct use of ground-truth target boxes during recognition.
The top two success rates in each column are highlighted in the boxed query results.}
\label{tab:main}
\begin{tabular}{c|cccccccc|cc}
\hline
\multirow{3}{*}{\textbf{Method}} & \multicolumn{8}{c|}{\textbf{Box query}} & \multicolumn{2}{c}{\textbf{Point query}} \\ \cline{2-11} 
 & \multicolumn{2}{c|}{\textbf{Easy}} & \multicolumn{2}{c|}{\textbf{Moderate}} & \multicolumn{2}{c|}{\textbf{Hard}} & \multicolumn{2}{c|}{\textbf{All}} & \multicolumn{2}{c}{\textbf{All}} \\ \cline{2-11} 
 & \multicolumn{1}{c|}{\textit{\textbf{top-1}}} & \multicolumn{1}{c|}{\textit{\textbf{top-3}}} & \multicolumn{1}{c|}{\textit{\textbf{top-1}}} & \multicolumn{1}{c|}{\textit{\textbf{top-3}}} & \multicolumn{1}{c|}{\textit{\textbf{top-1}}} & \multicolumn{1}{c|}{\textit{\textbf{top-3}}} & \multicolumn{1}{c|}{\textit{\textbf{top-1}}} & \textit{\textbf{top-3}} & \multicolumn{1}{c|}{\textit{\textbf{top-1}}} & \textit{\textbf{top-3}} \\ \hline\hline
{\texttt{Single-View}} (softmax) & \multicolumn{1}{c|}{60.2} & \multicolumn{1}{c|}{81.3} & \multicolumn{1}{c|}{53.9} & \multicolumn{1}{c|}{76.0} & \multicolumn{1}{c|}{45.9} & \multicolumn{1}{c|}{70.1} & \multicolumn{1}{c|}{55.3} & 77.8 & \multicolumn{1}{c|}{45.0} & 69.6 \\ \hline
{\texttt{Single-View}} (ours) & \multicolumn{1}{c|}{62.0} & \multicolumn{1}{c|}{81.2} & \multicolumn{1}{c|}{54.7} & \multicolumn{1}{c|}{74.9} & \multicolumn{1}{c|}{{\bf{51.5}}} & \multicolumn{1}{c|}{69.8} & \multicolumn{1}{c|}{57.0} & 76.6 & \multicolumn{1}{c|}{45.1} & 69.7 \\ \hline
{\texttt{Amodal-Rec}}~\cite{yang2019embodied} & \multicolumn{1}{c|}{59.4} & \multicolumn{1}{c|}{80.7} & \multicolumn{1}{c|}{51.9} & \multicolumn{1}{c|}{76.1} & \multicolumn{1}{c|}{43.3} & \multicolumn{1}{c|}{68.1} & \multicolumn{1}{c|}{53.6} & 76.6 & \multicolumn{1}{c|}{44.4} & 68.6 \\ \hline
{\texttt{Amodal-Rec}}~\cite{yang2019embodied} w/ {\texttt{Random}} & \multicolumn{1}{c|}{57.9} & \multicolumn{1}{c|}{79.7} & \multicolumn{1}{c|}{50.0} & \multicolumn{1}{c|}{75.9} & \multicolumn{1}{c|}{41.8} & \multicolumn{1}{c|}{68.8} & \multicolumn{1}{c|}{52.0} & 76.2 & \multicolumn{1}{c|}{43.4} & 68.7 \\ \hline
{\texttt{Amodal-Rec}}~\cite{yang2019embodied} w/ {\texttt{Fixation}} & \multicolumn{1}{c|}{57.4} & \multicolumn{1}{c|}{79.7} & \multicolumn{1}{c|}{49.7} & \multicolumn{1}{c|}{75.8} & \multicolumn{1}{c|}{42.9} & \multicolumn{1}{c|}{69.3} & \multicolumn{1}{c|}{51.9} & 76.2 & \multicolumn{1}{c|}{42.6} & 68.1 \\ \hline
Ours & \multicolumn{1}{c|}{{\bf{64.1}}} & \multicolumn{1}{c|}{{\bf{81.9}}} & \multicolumn{1}{c|}{{\bf{55.5}}} & \multicolumn{1}{c|}{{\bf{77.0}}} & \multicolumn{1}{c|}{48.2} & \multicolumn{1}{c|}{{\bf{71.0}}} & \multicolumn{1}{c|}{{\bf{57.9}}} & {\bf{78.2}} & \multicolumn{1}{c|}{{\bf{45.3}}} & {\bf{69.9}} \\ \hline
Ours w/ {\textit{G.T. tracking}} & \multicolumn{1}{c|}{{\bf{65.1}}} & \multicolumn{1}{c|}{{\bf{83.2}}} & \multicolumn{1}{c|}{{\bf{56.0}}} & \multicolumn{1}{c|}{{\bf{77.6}}} & \multicolumn{1}{c|}{{\bf{51.6}}} & \multicolumn{1}{c|}{{\bf{72.2}}} & \multicolumn{1}{c|}{{\bf{59.2}}} & {\bf{79.1}} & \multicolumn{1}{c|}{-} & - \\ \hline
\end{tabular}
% \vspace{-5pt}
\end{table*}


\begin{table}[t]
\centering
\scriptsize
\caption{\todo{Ablation studies about policies, the evidential fusion, and the uncertainty-aware reward. Add ours without fusion (Last-step, Vote).}}
    \label{tab:ablation}
    \begin{tabular}{c|c|c|c|cc}
    \hline
    \multirow{2}{*}{\textbf{Method}} & \textbf{Easy} & \textbf{Moderate} & \textbf{Hard} & \multicolumn{2}{c}{\textbf{All}} \\ \cline{2-6} 
     & \textit{\textbf{top-1}} & \textit{\textbf{top-1}} & \textit{\textbf{top-1}} & \multicolumn{1}{c|}{\textit{\textbf{top-1}}} & \multicolumn{1}{c}{\textit{\textbf{top-3}}} \\ \hline\hline
    Ours & {\bf{65.1}} & {\bf{56.0}} & {\bf{51.6}} & \multicolumn{1}{c|}{{\bf{59.2}}} & {\bf{79.1}} \\ \hline
    w/ {\texttt{Random}} & 62.1 & 49.6 & 38.2 & \multicolumn{1}{c|}{53.1} & 76.4 \\ \hline
    w/ {\texttt{Fixation}} & 63.7 & 55.2 & 51.0 & \multicolumn{1}{c|}{58.4} & 77.9 \\ \hline\hline
    w/ {\textit{Mean evidence}} & 64.6 & 55.3 & 49.4 & \multicolumn{1}{c|}{58.5} & 78.6 \\ \hline
    w/o $u^t$-aware reward & 64.8 & 55.4 & 43.0 & \multicolumn{1}{c|}{57.2} & 78.3 \\ \hline
    \end{tabular}
% \vspace{-5pt}
\end{table}



% \begin{minipage}{0.4\textwidth}
%     \centering
%     \includegraphics[width=1\linewidth]{figures/results/success_by_step.pdf}
%     \captionof{figure}{Performance between different agents over recognition steps.}
%     \label{fig:succ_by_step}
% \end{minipage}
% \vspace{2mm}
% \begin{minipage}{0.58\textwidth}
%     \centering
%     \scriptsize
%     \captionof{table}{Ablation studies about policies, the evidential fusion, and the uncertainty-aware reward.}
%     \begin{tabular}{c|c|c|c|cc}
%     \hline
%     \multirow{2}{*}{\textbf{Method}} & \textbf{Easy} & \textbf{Moderate} & \textbf{Hard} & \multicolumn{2}{c}{\textbf{All}} \\ \cline{2-6} 
%      & \textit{\textbf{top-1}} & \textit{\textbf{top-1}} & \textit{\textbf{top-1}} & \multicolumn{1}{c|}{\textit{\textbf{top-1}}} & \multicolumn{1}{c}{\textit{\textbf{top-3}}} \\ \hline\hline
%     Ours & {\bf{65.1}} & {\bf{56.0}} & {\bf{51.6}} & \multicolumn{1}{c|}{{\bf{59.2}}} & {\bf{79.1}} \\ \hline
%     w/ {\texttt{Random}} & 62.1 & 49.6 & 38.2 & \multicolumn{1}{c|}{53.1} & 76.4 \\ \hline
%     w/ {\texttt{Fixation}} & 63.7 & 55.2 & 51.0 & \multicolumn{1}{c|}{58.4} & 77.9 \\ \hline\hline
%     w/ {\textit{Mean evidence}} & 64.6 & 55.3 & 49.4 & \multicolumn{1}{c|}{58.5} & 78.6 \\ \hline
%     w/o $u^t$-aware reward & 64.8 & 55.4 & 43.0 & \multicolumn{1}{c|}{57.2} & 78.3 \\ \hline
%     \end{tabular}
%     \label{tab:ablation}
% \vspace{2mm}
% \end{minipage}

==> sec/0_abstract.tex <==
\begin{abstract}
Active recognition enables robots to intelligently explore novel observations, thereby acquiring more information while circumventing undesired viewing conditions.
Recent approaches favor learning policies from simulated or collected data, wherein appropriate actions are more frequently selected when the recognition is accurate.
However, most recognition modules are developed under the closed-world assumption, which makes them ill-equipped to handle unexpected inputs, such as the absence of the target object in the current observation.
To address this issue, we propose treating active recognition as a sequential evidence-gathering process, providing by-step uncertainty quantification and reliable prediction under the evidence combination theory.
Additionally, the reward function developed in this paper effectively characterizes the merit of actions when operating in open-world environments.
To evaluate the performance, we collect a dataset from an indoor simulator, encompassing various recognition challenges such as distance, occlusion levels, and visibility.
Through a series of experiments on recognition and robustness analysis, we demonstrate the necessity of introducing uncertainties to active recognition and the superior performance of the proposed method.
\end{abstract}

==> sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}
% 1. The area I’m working on and why it’s important.
Passive visual recognition, encompassing a broad range of approaches such as image-based and video-based techniques~\cite{yue2015beyond,he2016deep,dosovitskiy2020image,liu2022video}, has experienced tremendous success in recent decades.
Nonetheless, a contrasting approach, the active recognition system~\cite{aloimonos1988active,aloimonos1990purposive,ammirato2017dataset}, offers unique advantages.
Namely, it benefits from the ability to move within and perceive its environment, allowing it to dynamically determine visual inputs, as opposed to relying on pre-captured images.
% Namely, this engagement enables the agent to select the subsequent action, which in turn, significantly enhances recognition performance.

% Image- or video-based image recognition [] has achieved great success in the era of deep learning []. They are also called passive recognition [] since the image or video is pre-captured by the human and then input to a deep learning model to perform recognition. By comparison, in robot recognition, the robot itself has the ability to actively determine visual inputs on-the-fly, i.e., it has the ability to move to actively perceive the object-of-interest. In other words, the agent or other mobile platforms can choose different views to improve recognition performance. Such kind of recognition is termed active recognition (AR). Essentially, the agent interacts with the environment and then dynamically chooses the next action, where this recognition procedure will iterate sequentially. Recent active recognition research in embodied AI has done A, B, and C, and have achieved remarkable process.

% 2. The specific problem(s) I’m tackling.
% 3. Why those problems remain tricky with current technologies (i.e. why existing state-of-the-art isn’t quite enough).
A number of approaches~\cite{andreopoulos2013computational,atanasov2014nonmyopic,kasaei2018perceiving,bajcsy2018revisiting} in active recognition have been proposed over the years with information gain quantification~\cite{denzler2002information}, auxiliary task modeling~\cite{cheng2018geometry,ramakrishnan2018sidekick}, and discriminative feature discovery~\cite{jayaraman2016look}.
Given the sequential nature of active recognition, prevalent approaches~\cite{jayaraman2016look,ding2023learning,yang2019embodied,fan2021flar} involve combining recognition models, such as object detectors or classifiers, with reinforcement learning techniques.
The rewards, which can take the form of recognition accuracy or softmax probabilities, serve as incentives for the policy and are directly associated with the outputs of the recognition model.
Nevertheless, the reward could be misleading when deploying the agent in open-world scenarios~\cite{gallos2019active}.
For instance, consider an agent being queried with a target in the initial observation. The target may be out of view during subsequent movements, \ie, an unexpected input for the recognition system.
As a consequence, the recognition might fail to provide rewards that accurately represent the worth of actions being taken, impeding effective policy learning.

% 4. My new insight(s) / approach to solving the problem.
Regarding this challenge, our insight is derived from an instinctive understanding of how humans learn from experience. 
We consciously weigh our learning based on the level of trust we have in our observations. 
When faced with a high degree of uncertainty, we exercise caution in drawing conclusions from our experiences.
Likewise, the agent should evaluate the uncertainty in its observations to avoid being negatively influenced by unexpected inputs, such as when the target object exhibits high ambiguity or is simply not present in the input.

Besides, compared to passive recognition, the importance of modeling uncertainty is more prominent in active recognition, since the operating environment for agents is inherently open and unpredictable.
This area, however, remains under-explored as recent methods often resort to recognition models built under the closed-world assumption and then directly using softmax outputs as the confidence measure.
In this paper, we choose to model active recognition as a sequential evidence-gathering process, wherein the agent learns to explore trustworthy observations and gives the final prediction based on a collection of opinions.
The comparison of the proposed method with standard active recognition methods is depicted in Figure.~\ref{fig:overview}, where our agent can assign high uncertainties to inputs lacking target objects.
After actively exploring multiple views, the final prediction of the target is derived from a combination of collected opinions using Dempster-Shafer's combination theory~\cite{josang2016subjective}.
% In this approach, the higher the uncertainty, the less influence it exerts on the decision.

% 5. How I evaluate the new approach (i.e. how to convince the reader that this new approach is valuable).
% The task of previous active recognition methods usually following two streams. 
% The first does not specifically assign the target while regard the overall discovered objects in the scene.
% The second choose to manually select the target in the first frame with a bounding box.
% Our task formalization generally follows the second stream as we want the agent to recognize a specific object in the scene.
% However, we find the bounding box could be ambiguous on querying as the bounding box contains much background, especially dealing with snaky object shapes.
% And selecting a bounding box by human to query is also not intuitive.
% Our task choose to query object by pointing at the object (shown in Fig). It contains less ambiguity.
% The task is named point-query active recognition (PQ\textit{AR}).
% It makes the task more challenging due to two reasons. First, the query point could be located anywhere on the target object. Second, we have no clues of the shape and location of the target in the image.
Furthermore, to evaluate active recognition approaches, we collect a new dataset from an existing indoor simulator~\cite{szot2021habitat,savva2019habitat} where the target could be queried using a box or a point.
The motivation for introducing point query to active recognition lies in two aspects.
First, point queries can be less ambiguous, as bounding boxes inevitably include background elements, particularly when dealing with irregular target shapes. Second, querying by pointing is more aligned with human intuition.
In addition, each test instance in our dataset is accompanied by a recognition difficulty level, taking into account factors such as visibility, observed pixels, and distance.
We expect that the difficulty level will more effectively demonstrate the value of active recognition during evaluation, as the agent can potentially overcome these challenges, unlike in passive recognition.
% 6. Explicitly list the major contributions, i.e. “Our contributions are…” This can feel awkward and pedantic the first time you do it, but this helps reviewers evaluate your work (and they will look for it).

The primary contributions of this paper are as follows: (1) We develop a novel active recognition approach using evidence theory to address the challenges of open-world environments, which are largely overlooked by other methods. (2) We build a new dataset for evaluating active recognition agents, encompassing 13200 test instances across 27 different indoor object categories. Importantly, each test instance is assigned a recognition difficulty level for a more comprehensive assessment of methods. (3) We conduct extensive experiments and analyses of the proposed method and other baselines. These investigations demonstrate the trustworthiness and superior performance of our method.

% 7. Road map for the rest of the paper (so the reader can skip to sections of interest, if they so desire).

\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{figures/overview.pdf}
    \caption{An overview of active recognition agents operating in an open-world environment with different recognition models. The agent is initially queried to perform recognition. In standard practice, the recognition model is unable to identify its own failures, especially when confronted with unexpected inputs, which may lead to incorrect rewards for the policy. In contrast, our approach estimates uncertainty at each step and fuses the collected evidence to provide a final prediction.}
    \label{fig:overview}
\end{figure}
% ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~

==> sec/2_related_work.tex <==
\section{Related Work}
\label{sec:related_work}
% 1. Active recognition. Explain different rewards.
% 2. Uncertainty estimation. How to deal with open-world.
%   a. Dempster-Shafer theory in decision making,
%   b. Multi-view recognition.
\noindent{\bf{Active Recognition.}}
Embodied artificial intelligence, a long-standing field driven by enabling agents to learn through interactions, has been investigated across various streams~\cite{chaplot2020object,gadre2022continuous,kotar2022interactron,nilsson2021embodied}. 
As a notable branch, Active Recognition~\cite{aloimonos1990purposive,ballard1991animate,ammirato2017dataset,fang2020move,cheng2018geometry,gallos2019active,liu2018extreme} lets the agent explore observations with its own incentives, thereby achieving improved recognition performance.

Recent approaches~\cite{jayaraman2016look,fan2021flar,ding2023learning,yang2019embodied} in active recognition typically represent the recognition as a Markov Decision Process and rely on Reinforcement Learning (\textit{RL}) to learn moving strategies from interactions.
Unlike other \textit{RL} scenarios where the reward function is explicitly specified by the environment~\cite{mnih2016asynchronous,schulman2017proximal}, the reward function in active recognition is associated with the recognition module, which is defined as information gain~\cite{liu2018extreme}, the recognition accuracy~\cite{jayaraman2016look,jayaraman2018end,cheng2018geometry,yang2019embodied}, or the recognition score~\cite{ammirato2017dataset,ding2023learning}. 
In~\cite{jayaraman2016look,ramakrishnan2019emergence}, the authors propose an active recognition agent with modules to aggregate historical information and predict the next views. The policy learning is supervised by a binary reward function checking whether the top prediction is correct.
In parallel, \cite{ding2023learning} selects the surrogate reward, defined as the detection score, during policy learning.

However, these reward definitions might not adequately reflect the value of actions when the agent encounters unexpected visual inputs, especially when the target is absent from the current frame. 
This is because the recognition model was developed within a closed-world setting.
Improper rewards can compromise the resulting recognition policy after training. 
To address this, we introduce uncertainty estimation into the active recognition process. 
This ensures the agent updates its policy only when it performs recognition with confidence.


% when deploying the agent to open environments, as no uncertainties are estimated.

% The reward function is the value indicator of the action being selected during the policy training. 

% They study the policy on view selection by conducting the experiments in a relatively constrained environment that the target is placed at the center of viewing sphere.
% \cite{yang2019embodied} pays attention to a more challenging scenario by developing \textit{AR} agents in indoor environments, where the agent can freely move to recognized the target.

% In parallel, \cite{ding2023learning} models \textit{AR} with Decision Transformer, and employs the agent in an indoor simulator.
% Previous \textit{AR} methods can be primarily identified into two groups considering whether the agent operates in an open environment.
% For the method studying \textit{AR} in a closed-world~\cite{}, the input to the agent always contains the target object, like the robot is always looking at and rotating   

\noindent{\bf{Uncertainty Estimation.}} Conventional visual recognition models are unable to identify their own failures. Nonetheless, this ability could be essential when it comes to real-world applications, particularly for embodied agents. Bayesian neural networks~\cite{gal2015bayesian,dusenberry2020efficient,kristiadi2020being,kwon2020uncertainty} equip the recognition models predicting uncertainties as the mutual information between data and parameters. In stark contrast, Evidential Deep Learning~\cite{amini2020deep,sensoy2018evidential} established on the Dempster-Shafer Theory has been investigated in different applications~\cite{bao2021evidential,corbiere2021beyond,han2022trusted}, which learn the prior of the categorical prediction directly. Inspired by the success of uncertainty quantification of evidential approaches, the proposed method formulates active recognition as a sequential multi-source evidence fusion under the same frame of discernment. With this modeling, we can more effectively combine knowledge in consecutive observations and handle open-world challenges.


% ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~

==> sec/3_task.tex <==
\section{Task Settings and Notations}
\label{sec:task}
% 1. Task definition. 
% 2. Why do we choose point over bounding boxes?
%   Advantages:
%   a. More intuitive interaction.
%   b. Fewer ambiguities. Does not contain bg. The pixel-level label is unique.
%   Challenges:
%   a. Location and shape of object unknown.
%   b. Dealing with thin objects, like door frames.
We describe our setting by deploying the active object recognition agent in an indoor environment. 

The recognition agent is spawned at a location in an indoor environment without prior knowledge about the scene, {\it{e.g.}}, the map. At the initial timestep $t=1$, the agent is queried with a target $x$ in the current visual observation $v^1$, either selected by a bounding box $q^{box}_x$ or a point $q^{point}_x$. And a total of $T$ timesteps is allowed for the agent to obtain the final prediction of the target category. Besides the final step, the agent could take an additional action $a^t\in\mathcal{A}$ at $t=1,\dots,T-1$ to change its viewing point, where $\mathcal{A}$ is the action space. By taking movements, the agent could improve its recognition performance by collecting information and give the final predicted label $\hat{y}$ at $t=T$. It is worth noting that the setting could be smoothly generalized to other simulators and different types of targets, like active scene recognition~\cite{xiao2012recognizing,jayaraman2016look,ramakrishnan2021exploration,fan2021flar}.

To provide details about our setup, the observation $v$ is captured by an RGB camera mounted at the height of $1$ meter above the ground, featuring a height-by-width resolution of $640\times800$. The action space is defined as $\mathcal{A}=\{{\texttt{move\_forward}}, {\texttt{turn\_left}}, {\texttt{turn\_right}}, {\texttt{look\_up}},\\{\texttt{look\_down}}\}$. 
The agent is allowed to move $0.25$m, turn $10$ degrees, or tilt $10$ degrees for different actions.
Previous works on active recognition~\cite{ding2023learning,yang2019embodied} usually do no contain {\texttt{look\_up}} and {\texttt{look\_down}} in to their action space. This may potentially compromise the agent's performance, particularly in the case of objects situated at higher locations in the observation.
As the agent forms multi-round interactions with the environment, the objective of an effective approach lies in three major components, including visual classification, information aggregation, and intelligent moving policies, which we will elaborate on in later sections.

% ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~

==> sec/4_method.tex <==
\section{Evidential Active Recognition}
\label{sec:method}
% 1. How do we undestand active recognition?
% 2. What's the difference with previous softmax-based approaches? What happens to other methods if we deploy the agent to real world.
% 3. How do we calculate per-frame evidence? How to model it?
% 4. Why evidence fusing is important? And why do we choose late fusion (we want per-frame prediction to be independent as missing could happen anywhere in a sequence)?
In this section, we introduce a model called Evidential Active Recognition, which is designed to address the challenges associated with developing agents in an open-world context. 
We comprehend active recognition as an evidence-collecting procedure in which the agent explores and gathers knowledge to make predictions.
Evidence for each class is estimated on a per-step basis, complemented by an additional term that describes the overall uncertainty.
Intuitively, as the agent freely moves in the environment, uncertainty appears when the target is absent, or when the viewpoint is not optimal for acquiring discriminative features.
To capture the uncertainty, the Dirichlet prior is placed for known classes~\cite{sensoy2018evidential} to provide trustworthy results.
In comparison to active recognition approaches that utilize softmax outputs, the estimated uncertainty then plays a key role in policy learning by redefining the reward function.
The final multinomial opinion on the target category follows the Subject Logic~\cite{barnett2008computational,josang2016subjective} to fuse evidence from different views at the last step.

\subsection{Preliminaries}
Current visual recognition models often rely on the softmax operator to give probabilities.
Nonetheless, as the probability is normalized, it could lead to overconfident predictions or even failures when handling unknown inputs. 
Evidential deep learning approaches~\cite{sensoy2018evidential}, on the contrary, choose to develop uncertainties under the scheme towards subjective probabilities~\cite{barnett2008computational,josang2016subjective}. For the next paragraph, we will start by introducing the formulation of evidential deep learning.

For a $K$-class recognition task, the frame of discernment $\Theta=\{k, 1\leq k\leq K\}$ contains $K$ exclusive singletons, {\it{e.g.}}, class labels.
Considering the visual observation $v^t$ at timestep $t$, we measure the mass in mutually exclusive propositions with a belief function $b_k^t$ leveraging the Dempster-Shafer Theory of Evidence (DST)~\cite{barnett2008computational}.
By providing an overall uncertainty mass $u^t$, these $K+1$ mass values satisfy
\begin{equation}
    \sum_{k=1}^K b_k^t+u^t=1, \quad 0\leq u^t,b_k^t\leq 1.
    \label{eq:belief_sum}
\end{equation}
% where $0\leq u^t,b_k^t\leq 1$.
The evidence $e^t_k$ is defined as the support evidence collected from the current observation $v^t$ to $k^{th}$ singleton. To form the opinion, the evidence $e^t_k$ is introduced to associate the belief function with Dirichlet distribution parameters $\alpha_k^t$ by
% To form the opinion, the evidence $e^t_k$, referring to the support evidence collected from the current observation $v^t$ to $k^{th}$ singleton, is introduced to associate the belief function with Dirichlet distribution parameters $\alpha_k^t$ by
\begin{equation}
    b^t_k=\frac{e^t_k}{S^t} \; {\textnormal{ and }} \; u^t=\frac{K}{S^t},
    \label{eq:belief_unc}
\end{equation}
where $S^t=\sum^K_{k=1}\alpha_k^t=\sum^K_{k=1}(e^t_k+1)$. As the conjugate prior for the multinomial distribution, the Dirichlet distribution characterized by $\alpha^t=[\alpha_1^t,\dots,\alpha_K^t]$ is then used to derive the subject opinion, \ie, the belief function as $b_k^t={e_k^t}/{S^t}$. 
Accordingly, the overall uncertainty $u^t$ arises if no significant evidence is being collected from known classes.

From the DST, the masses defined in Equation.~\ref{eq:belief_sum} is a reduction from the general hyper-opinion set $2^\Theta=\{\emptyset, 1, \dots, K, \{1, 2\}, \dots, \Theta\}$ that contains intimidating $2^K$ propositions. As no mass is assigned to the empty-set proposition, \ie, $b_{\emptyset}^t=0$, the uncertainty $u^t$ is consequently the summation of contained non-singleton belief masses. Namely, the overall uncertainty $u^t$ could be interpreted as the sum of conflicting evidence occurring between 2 or more classes, which could be formulated as
\begin{equation}
    u^t=1-\sum_{k=1}^K b_k^t=\sum_{P,P\in2^\Theta,2\leq |P|\leq K} b_P^t,
    \label{eq:uncertainty}
\end{equation}
where we use $P$ as the symbol for any proposition, and it satisfies $0\leq b_P^t\leq 1$.

\subsection{Evidence Fusion}
% 1. The challenge in evidence combination
% 2. Why late fusion?
After discussing belief and uncertainty for a single-step observation, we now proceed to explore how to fuse evidence among multiple predictions.
Two primary fusion strategies are employed in active recognition. The first one is early fusion~\cite{yang2019embodied,jayaraman2016look}, which recurrently aggregates temporal visual information at the feature level. The second one is late fusion, which involves techniques such as voting or averaging the softmax outputs~\cite{ding2023learning}.
% Two primary fusion strategies are employed in active recognition, \ie, early fusion~\cite{yang2019embodied,jayaraman2016look}, which recurrently aggregates temporal visual information at the feature level, and late fusion, which involves techniques such as voting or averaging the softmax outputs~\cite{jayaraman2016look,ding2023learning}.
We propose fusing per-step evidence within the framework of subjective probabilities~\cite{josang2016subjective}, which can be considered as a form of late fusion.

The insights of doing late fusion are three-fold. First, the unexpected visual input can occur at any timestep during a recognition episode, regardless of whether it takes place during policy training or testing. 
Thus, the feature could be contaminated if it is aggregated at an early stage, and difficult to differentiate at which time the recognition uncertainty is introduced.
This, in turn, impedes the provision of reasonable rewards for evaluating the policy.
Second, late fusion better accommodates the assumption in DST that available evidence from different sources should be independently measured.
Third, compared to recurrently fusing temporal features, the late fusion is unaffected by the order of visual observations.
Considering a group of visual observations, the recognition result should remain unchanged by the order in which they are presented.
% Advantage: 1. interpretability. 2. Independent

With no loss of generality, we formulate the evidence combination between any two basic belief functions $b_k^t,b_k^j$ on different observations under the same frame of discernment, \ie, $\Theta$, as:
\begin{equation}
\begin{split}
    b_k&=b_k^t\oplus b_k^j=\frac{1}{\sum_{P^t\cap P^j\neq\emptyset}b_{P^t}^t b_{P^j}^j}\sum_{P^t\cap P^j=k} b_{P^t}^t b_{P^j}^j \\
    &=\frac{b^t_k b^j_k + b^t_k u^j + b^j_k u^t}{1-\sum_{i\neq q}b^t_i b^j_q},
\end{split}
\end{equation}
where $P^t$ and $P^j$ are any two propositions in $2^\Theta$.
Similarly, the uncertainty after the combination is defined as $u=u^tu^j/({1-\sum_{i\neq q}b^t_i b^j_q})$, where the denominator serves as a normalization factor, representing the total valid mass.
It should be noted that the combination reduces conflicting evidence as one single term, \ie, approximate with the uncertainty $u^t$ and $u^j$ as in Equation.~\ref{eq:uncertainty}, to lower the computation complexity.
Moreover, this combination guarantees the final prediction to be more strongly influenced by the belief assignment with lower uncertainty.

Subsequently, given a sequence of $T$ observations collected by the agent, we can derive the final belief function by
\begin{equation}
    b_k=b_k^1\oplus b_k^2\oplus \dots \oplus b_k^T.
\end{equation}
The combination inherently adheres to the commutative property, implying that the order of observations does not impact the outcomes. And the final prediction of the category is $\hat{y}=\arg\max_{k}b_k$.

\subsection{Developing Opinions}
% 1. Independent between frames, so we can do evidence fusion. The DS theory requires two sets of masses to be independent to do fusion.
In this section, we outline how to develop opinions for the visual recognition model using training data. 
The deep recognition model used in our approach could be generally denoted as a mapping function $f_{\theta}(\cdot)\rightarrow\mathbb{R}$ with a set of parameters, \ie, $\theta$.
The output of the recognition model is obtained directly from the current input as evidence $e_k, 1\leq k\leq K$ after applying a non-negative function, such as an exponential function or sigmoid.
Following evidential deep learning~\cite{sensoy2018evidential}, the training is implemented as the evidence acquisition on a Dirichlet prior, whose loss is formulated as
\begin{equation}
    \mathcal{L}_{edl}^t=\sum^K_{i=1}y_{i}[\log(\sum^K_{j=1}\alpha_{j}^t)-\log(\alpha_{i}^t)],
\end{equation}
where $\mathbf{y}=[y_1, \dots, y_{i}, \dots, y_{K}]^T$ is the one-hot label, and $\bm{\alpha}^t=[\alpha_1^t, \dots,\alpha_{i}^t,\dots, \alpha_{K}^t]$ with $\alpha_{i}^t=e_i^t+1$ are parameters of a Dirichlet distribution $Dir(\cdot|\bm{\alpha})$.
Additionally, a Kullback-Leibler loss is incorporated to promote mutual exclusivity among singleton beliefs, defined as
\begin{equation}
    \mathcal{L}_{kl}^t=\textit{KL}(Dir(\cdot|\tilde{\bm{\alpha}}^t)||Dir(\cdot|\langle 1, \dots, 1\rangle)),
\end{equation}
where $\tilde{\bm{\alpha}}^t=\mathbf{y}+(1-\mathbf{y})\odot\bm{\alpha}^t$, and $\odot$ is for element-wise multiplication. Combining all terms, the total loss for an observation $v^t$ is
\begin{equation}
    \mathcal{L}^t=\mathcal{L}_{edl}^t + \lambda_{kl}\mathcal{L}_{kl}^t,
\end{equation}
where $\lambda_{kl}$ is an annealing weight to gradually increase the effect of $\mathcal{L}_{kl}^t$.

Although the combination rule provides results based on multiple observations, we opt to train our recognition model using single observations only.
The rationale behind this choice is that if all observations contain the target to be recognized, adding another loss on fused evidence does not alter the optimality of the loss function. Conversely, if the target is missing in any observations, the training may be adversely impacted.


\subsection{Uncertainty-aware Policy Learning}
\begin{figure*}[t]
    \centering
    \includegraphics[width=1\linewidth]{figures/method_3.pdf}
    \caption{An illustration of a recognition episode and the proposed agent's architecture in the grey box. We select three frames ($t=1,4,10$) along with their estimated opinions. The bars for top prediction and uncertainty are colored green and red, respectively. Note that uncertainty arises when the target is partially out of view at the first step. Despite this, the final result is accurate due to the fusion of evidence.}
    \label{fig:method}
\end{figure*}

The overall architecture of our proposed agent is demonstrated in Figure.~\ref{fig:method}.
Besides the recognition model to predict the category of the target, the policy module $\pi_{\phi}(a^t|s^{t-1})$ with parameters $\phi$ is supposed to control the robot to maximize the accumulated reward $R=\sum_{t=2}^T r^t$.
The state $s^{t-1}$ describes the aggregated information from observations till the timestep $t-1$.
To prevent interference with the recognition, we use a separate recurrent unit $g(\cdot)$ for fusing temporal knowledge.
The state is then expressed as $s^{t}=g(v^1,\dots,v^{t},q_x^t)$, where $q_x^t$ denotes the binary mask of the target $x$ at timestep $t$.
To ensure clarity in our study and to eliminate uncertainties introduced by other modules, the mask $q_x^t$ is derived from the ground-truth bounding box of the target, consistent with previous embodied perception works~\cite{zhao2023zero,wortsman2019learning,pal2021learning}. 
In practical applications, the agent can utilize off-the-shelf class-agnostic visual trackers~\cite{wang2019fast} to obtain $q_x^t$.
% The mask $q_x^t$ is acquired from an off-the-shelf class-agnostic visual tracker~\cite{wang2019fast} and could be replaced by other tracking approaches.

We design a novel reward to stabilize policy learning, especially when the target is missing in the observation.
According to our prediction result as in Equation~\ref{eq:belief_unc}, the reward $r^t$ should reflect the evidence of the correct class.
To this end, the proposed reward is straightforwardly defined as $r^t=b^t_y$.
Note that we use $b^t_y$ to represent the belief for the correct class, which can also be interpreted as the normalized evidence.
The reward $r^t$ varies between 0 to 1 depending on how much the recognition model collects the evidence for the target class.
Since our output includes an uncertainty term, the belief for all known classes may be extremely low when encountering an unknown input, suggesting that the action leading to the observation should not be rewarded.

As discussed in~\cite{fan2023avoiding,yang2019embodied}, joint training of the recognition module and the policy can lead to a collapsed outcome. 
This is because an insufficiently-trained recognition model may not provide accurate rewards during the early training stages. 
Therefore, we perform a staged training: first, we train the recognition model using a heuristic policy, and then we train only the policy part using PPO~\cite{schulman2017proximal}, while keeping the recognition model fixed.


% ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~

==> sec/5_dataset.tex <==
\section{Testing Dataset for Active Recognition}
\label{sec:dataset}

\begin{figure}[t]
    \centering
        \includegraphics[width=1\linewidth]{figures/ds_example_2.pdf}
        \includegraphics[width=0.9\linewidth]{figures/difficulty_cat.pdf}
    \caption{We present an example of test data from the proposed dataset on the left. The target object is covered by a green mask, allowing for point or box queries during testing. The target (in this case, a picture) is both occluded by the wall and partially out-of-view, thus visibility is calculated as the ratio of observed pixels to total pixels belonging to the target. On the right, the distribution of difficulty levels across all categories is depicted.}
    \label{fig:dataset}
\end{figure}
% 1. Explain why do we need to build a dataset
%   a. We are building the testing data. The motivtion of active recognition is to avoid undesired viewing conditions.
%   b. How do we collect data, and why choose this dataset? There is no overlap between training and testing scenes.
%   c. Statistcs.
Compared to passive recognition, active recognition is motivated to avoid undesired viewing conditions, including but not limited to heavy occlusions and the out-of-view, where adjusting viewpoints is urgent and inevitable. To better evaluate active recognition approaches, we build a testing dataset designated for assessing their performances under different recognition challenges, which is collected from the current simulator MP3D~\cite{chang2017matterport3d,savva2019habitat,szot2021habitat}. 

The testing dataset from MP3D~\cite{chang2017matterport3d} contains 90 building-scale indoor spaces covering diverse scene categories. 
For each test instance, the agent's starting position and the query are randomly specified, ensuring that the relative distance between them falls within the range of 3 to 6 meters.
Since the semantic annotation in MP3D~\cite{chang2017matterport3d} could be noisy, we manually remove erroneous or low-quality queries, resulting in a total of $13200$ testing instances.
The training of the agent is conducted using the non-overlapping HM3D dataset~\cite{ramakrishnan2021hm3d}, which contains 145 semantically-annotated indoor scenes, along with randomly generated initial positions and queries.

% 2. Observation and action space
% \noindent{\bf{Observation and Action.}} 


% 3. Objects categories
\noindent{\bf{Object categories.}} We select $27$ object categories from over $40$ labeled classes that exists in both datasets~\cite{chang2017matterport3d,ramakrishnan2021hm3d}. A category is selected only if it does not contain high ambiguities (objects, misc, {\it{etc}}.) or belongs to building components (wall, ceiling, stairs, {\it{etc}}.).

% 4. How to define difficulty
%   a. The visibility is defined by three aspects: the relative location (the iniital location, the viewpoint, the distance), the occlusion and the character of the target itself.
%   b. Our criteria to define difficulty.
\noindent{\bf{Recognition difficulty.}} We introduce an estimate of recognition difficulty for each testing instance. Unlike~\cite{yang2019embodied}, we evaluate the difficulty level from three perspectives: {\it{visibility}}, {\it{relative distance}}, and {\it{observed pixels}}. {\it{Visibility}} is determined by the ratio computed by dividing the unoccluded segmentation mask of the target by its observed mask. 
To consider partially out-of-view conditions, the unoccluded mask is captured within an enlarged viewing window.
An example of a test instance is depicted on the left side of Figure.~\ref{fig:dataset} where the target object is not entirely within the agent viewing window and is additionally occluded by a wall.
The second aspect, {\it{relative distance}}, measures the distance between the agent and the target object.
This is determined by subtracting the normalized relative distance (originally ranging from 3 to 6 meters) from 1.
{\it{Observed pixels}} account for the visible pixels of the target object and are normalized with a cap at 102400 pixels.
The final difficulty score combines these three factors using weights of 0.2, 0.2, and 0.6, respectively. We emphasize {\it{observed pixels}} because the other two aspects might not sufficiently represent the recognition challenges posed by tiny objects.

The difficulty level is assigned as follows: "hard" if the score is less than 0.33, "moderate" if it falls between 0.33 and 0.66, and "easy" for all other cases.
The difficulty level for each category is depicted on the right of Figure.~\ref{fig:dataset}.
Since we do not re-balance or re-sample rare classes, the category distribution follows a long-tail pattern, reflecting their true occurrences in testing scenes.
The dataset will be made publicly available to facilitate reproducible research comparisons.
More detailed dataset generation and statistics can be found in the supplementary.

% The total system is defined as a function on $x$ to $y$.
% ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~

==> sec/6_experiment.tex <==
\section{Experiments}
\label{sec:experiment}
% To validate the performance of our method, we have three primary objectives to fulfill in this section. 
% The first aspect involves active recognition results. 
To validate the effectiveness of our method, we first compare the proposed method with other approaches using our new dataset, demonstrating the benefits of uncertainty-aware policy learning and evidence fusion.
Next, we examine the behavior of provided uncertainties across various dimensions, such as categories, steps, and recognition difficulties.
More experiments, including ablation studies, are conducted in the final part to further evaluate our method.

\subsection{Implementations}
% We need tracker, network architecture.
% 1. Only ten steps are used.
% 2. Action space and Observation space.
% 3. Network architectures.
% 4. Staged training and hyperparameters.
The recognition model, based on Faster R-CNN~\cite{ren2015faster}, is modified by replacing the region proposal network with the query box at the current timestep.
The backbone is ResNet-50~\cite{he2016deep} pretrained on the ImageNet~\cite{russakovsky2015imagenet}.
We use the ROI features with a C4 head~\cite{ren2015faster} and also fix the first three residual blocks during training as in~\cite{yang2019embodied}.
The training of the recognition model is accompanied by a heuristic fixation policy, which attempts to make movements that position the target at the center of the view.
Furthermore, the target is directly provided by the ground-truth bounding box at all timesteps.

The policy part is trained with the recognition model held fixed.
The policy network comprises an independent visual encoder, a single-layer Gated
Recurrent Unit (GRU) to integrate temporal knowledge, and two single linear-layer to perform as actor and critic on the GRU's output. 
% We use PPO~\cite{schulman2017proximal} to train policies with $\gamma=0.99$ and $\tau=0.95$ during the computation of returns.
For detailed architecture and other training hyper-parameters, please refer to our supplementary.

\subsection{Baselines}
% 1. Yang's method. Explain the reimplementation.
% 2. Single view, Random, Fixation, Approaching
The compared baselines serve two purposes, \ie, to demonstrate the effectiveness of incorporating intelligent strategies into the recognition process, and to highlight the advantages of modeling uncertainties in active recognition.
Heuristic recognition policy baselines, including {\textit{Single view}}, {\textit{Random}}, and {\textit{Fixation}}, employ a similar network architecture as other compared methods, but with alterations to the policy and the removal of uncertainty estimation.

\noindent{\textit{Single view}}: It imitates conventional passive recognition models that could not intelligently perceiving the target. It uses the initial observation for prediction.

\noindent{\textit{Random}}: The policy randomly selects an action at each step.

\noindent{\textit{Fixation}}: This policy aims to center the target within the view, potentially reducing undesired out-of-view conditions.

Furthermore, we re-implement Embodied-AR~\cite{yang2019embodied} which uses an additional convolutional GRU to recurrently aggregate visual features and generate predictions using softmax probabilities.
To ensure a fair comparison, we replace the training method in Embodied-AR~\cite{yang2019embodied} from REINFORCE~\cite{sutton1998introduction} to PPO~\cite{schulman2017proximal} and also the perception part from Mask R-CNN~\cite{he2017mask} to Faster R-CNN~\cite{ren2015faster}, aligning it with our approach.

\subsection{Performance Evaluation}
% 1. Metrics. Top-k evaluation (query could be ambiguous, like a cushion on a bed).
% 2. Active recognition success rate by difficulty (all, easy, moderate, hard).
% 3. By-step recognition performance (success rate, uncertainty, distance).
% 4. Example showing the recognition episodes (evolving uncertainty).
% 5. Perturbation happens (occlusion, motor failure).
% 6. The correlation between uncertainty and failed recognition.
% 7*. By step statistics:
%   a. Distance change by step.
%   b. Pixel visibility change by step.
%   c. Uncertainty change by step.
%   d. Action distribution by step.
% 8. (Supp) By category result.
%   a. By category uncertainty.
% 9. (Supp) Action distribution by steps.
\begin{table*}[t]
\centering
\footnotesize
\caption{Recognition success rate on the proposed dataset. 
% The results are reported based on predictions made at the final step. 
{\textit{Random}} and {\textit{Fixation}} two heuristic policies, while {\textit{G.T. tracking}} implies the direct use of ground-truth target boxes during recognition.
The top two success rates in each column are highlighted in the boxed query results.}
\label{tab:main}
\begin{tabular}{c|cccccccc|cc}
\hline
\multirow{3}{*}{\textbf{Method}} & \multicolumn{8}{c|}{\textbf{Box query}} & \multicolumn{2}{c}{\textbf{Point query}} \\ \cline{2-11} 
 & \multicolumn{2}{c|}{\textbf{Easy}} & \multicolumn{2}{c|}{\textbf{Moderate}} & \multicolumn{2}{c|}{\textbf{Hard}} & \multicolumn{2}{c|}{\textbf{All}} & \multicolumn{2}{c}{\textbf{All}} \\ \cline{2-11} 
 & \multicolumn{1}{c|}{\textit{\textbf{top-1}}} & \multicolumn{1}{c|}{\textit{\textbf{top-3}}} & \multicolumn{1}{c|}{\textit{\textbf{top-1}}} & \multicolumn{1}{c|}{\textit{\textbf{top-3}}} & \multicolumn{1}{c|}{\textit{\textbf{top-1}}} & \multicolumn{1}{c|}{\textit{\textbf{top-3}}} & \multicolumn{1}{c|}{\textit{\textbf{top-1}}} & \textit{\textbf{top-3}} & \multicolumn{1}{c|}{\textit{\textbf{top-1}}} & \textit{\textbf{top-3}} \\ \hline\hline
{\textit{Single view}} (softmax) & \multicolumn{1}{c|}{60.2} & \multicolumn{1}{c|}{81.3} & \multicolumn{1}{c|}{53.9} & \multicolumn{1}{c|}{76.0} & \multicolumn{1}{c|}{45.9} & \multicolumn{1}{c|}{70.1} & \multicolumn{1}{c|}{55.3} & 77.8 & \multicolumn{1}{c|}{45.0} & 69.6 \\ \hline
{\textit{Single view}} (ours) & \multicolumn{1}{c|}{62.0} & \multicolumn{1}{c|}{81.2} & \multicolumn{1}{c|}{54.7} & \multicolumn{1}{c|}{74.9} & \multicolumn{1}{c|}{{\bf{51.5}}} & \multicolumn{1}{c|}{69.8} & \multicolumn{1}{c|}{57.0} & 76.6 & \multicolumn{1}{c|}{45.1} & 69.7 \\ \hline
Embodied-AR~\cite{yang2019embodied} & \multicolumn{1}{c|}{59.4} & \multicolumn{1}{c|}{80.7} & \multicolumn{1}{c|}{51.9} & \multicolumn{1}{c|}{76.1} & \multicolumn{1}{c|}{43.3} & \multicolumn{1}{c|}{68.1} & \multicolumn{1}{c|}{53.6} & 76.6 & \multicolumn{1}{c|}{44.4} & 68.6 \\ \hline
Embodied-AR~\cite{yang2019embodied} w/ {\textit{Random}} & \multicolumn{1}{c|}{57.9} & \multicolumn{1}{c|}{79.7} & \multicolumn{1}{c|}{50.0} & \multicolumn{1}{c|}{75.9} & \multicolumn{1}{c|}{41.8} & \multicolumn{1}{c|}{68.8} & \multicolumn{1}{c|}{52.0} & 76.2 & \multicolumn{1}{c|}{43.4} & 68.7 \\ \hline
Embodied-AR~\cite{yang2019embodied} w/ {\textit{Fixation}} & \multicolumn{1}{c|}{57.4} & \multicolumn{1}{c|}{79.7} & \multicolumn{1}{c|}{49.7} & \multicolumn{1}{c|}{75.8} & \multicolumn{1}{c|}{42.9} & \multicolumn{1}{c|}{69.3} & \multicolumn{1}{c|}{51.9} & 76.2 & \multicolumn{1}{c|}{42.6} & 68.1 \\ \hline
Ours & \multicolumn{1}{c|}{{\bf{64.1}}} & \multicolumn{1}{c|}{{\bf{81.9}}} & \multicolumn{1}{c|}{{\bf{55.5}}} & \multicolumn{1}{c|}{{\bf{77.0}}} & \multicolumn{1}{c|}{48.2} & \multicolumn{1}{c|}{{\bf{71.0}}} & \multicolumn{1}{c|}{{\bf{57.9}}} & {\bf{78.2}} & \multicolumn{1}{c|}{{\bf{45.3}}} & {\bf{69.9}} \\ \hline
Ours w/ {\textit{G.T. tracking}} & \multicolumn{1}{c|}{{\bf{65.1}}} & \multicolumn{1}{c|}{{\bf{83.2}}} & \multicolumn{1}{c|}{{\bf{56.0}}} & \multicolumn{1}{c|}{{\bf{77.6}}} & \multicolumn{1}{c|}{{\bf{51.6}}} & \multicolumn{1}{c|}{{\bf{72.2}}} & \multicolumn{1}{c|}{{\bf{59.2}}} & {\bf{79.1}} & \multicolumn{1}{c|}{-} & - \\ \hline
\end{tabular}
% \vspace{-5pt}
\end{table*}

% 1. We fix the total recognition steps among different methods to $T=10$ for a fair comparison.
% 2. The success rate is reported by the last step for different agents.
% 3. why single view (yang) is better
% 4. why our (tracking) in hard does not met single view, always occluded, very far, hard to track, making movemenet does not bring much benefit to these hard samples.

% In this section, we present a quantitative comparison of performance metrics across different active recognition models, as shown in Table~\ref{tab:main}. 
In this section, we present a quantitative comparison across different active recognition models under various evaluation metrics. 
In line with established protocols~\cite{jayaraman2016look,yang2019embodied}, we set a limit of $T=10$ total allowed steps and subsequently report the performance at the final step.
% , which ensures a fair comparison among the methods under consideration.
We demonstrate the results for two distinct query types: box query and point query. The point query, in particular, poses a greater challenge as it does not deliver any information regarding the object's shape or its precise location.
Additionally, we provide the success rate across varying levels of recognition difficulty.

As shown in Table.~\ref{tab:main}, the aggregation of temporal information at the feature level encounters challenges when deployed in open-world environments. This finding stems from a comparison of the results derived from Embodied-AR~\cite{yang2019embodied} with a trained policy versus the {\textit{Single view}} (softmax) approach.
Step-by-step results for Embodied-AR~\cite{yang2019embodied} are depicted in Figure~\ref{fig:succ_by_step}, revealing a downward trend in recognition as more steps are taken. 
We postulate two potential reasons for this observed phenomenon.
Firstly, Embodied-AR~\cite{yang2019embodied} collates whole-image features across varying frames and subsequently leverages the initial query location to pool regional information from the aggregated feature for classification. 
As the agent alters its viewpoints, the regional feature may lose its discriminative power as the same queried region incorporates irrelevant information in subsequent frames.
Secondly, our dataset presents greater challenges compared to the one used in Embodied-AR~\cite{yang2019embodied}, primarily due to increased freedom of movement, \ie, the ability to look up and down. 
Consequently, the likelihood of the same queried region pertaining to the same object between consecutive frames diminishes.
These observations underscore the jeopardy of overlooking the inherent challenges posed by active recognition in open-world environments.

Another key observation from Table~\ref{tab:main} pertains to the results associated with the box query of "hard" level. Our result, using an off-the-shelf tracker~\cite{wang2019fast}, becomes less effective than {\textit{Single view}} approach but shows improved performance when utilizing ground-truth tracking.
This outcome can be attributed to the fact that the "hard" testing instances are typically subject to heavy occlusions and long distances, conditions under which the tracker often fails to locate the target beyond the initial view. 
This explanation also applies to the results of the point query, where tracking extremely small targets across multiple steps proves to be a challenging endeavor.

% random: a surge at step=2
The success rate over steps is depicted in Figure~\ref{fig:succ_by_step}. 
Overall, the proposed method shows an improvement in performance as more observations are taken, eventually reaching a saturation point.
Interestingly, there is a noticeable performance surge at $t=2$ for Ours w/ {\textit{Random}}. 
This can be attributed to the high probability of the target existing within the observation after a single movement. 
In essence, the proposed evidence fusion strategy can enhance recognition if the target is observable. Moreover, significant improvements can be achieved through the implementation of our uncertainty-aware policy learning approach.

\subsection{Uncertainty in Active Recognition}
% 1. Assigning unknown targets. Show uncertainty. Show behavior.
% 2. Miss the target during recognition.
% 3. Operate in open scenarios. Compare uncertainty.
\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\linewidth]{figures/results/uncertainty_by_diff.pdf}
    \includegraphics[width=0.8\linewidth]{figures/results/uncertainty_by_step.pdf}
    % \subfigure[Uncertainty and success rate by difficulty.]{
    %     \includegraphics[width=0.98\linewidth]{figures/results/uncertainty_by_diff.pdf}
    % }
    % \subfigure[Trends in uncertainty and success rate.]{
    %     \includegraphics[width=0.46\linewidth]{figures/results/uncertainty_by_step.pdf}
    % }
    % \vspace{-8pt}
    \caption{The change of uncertainties with respect to different difficulty levels and steps.}
    \label{fig:uncertainty}
% \vspace{-12pt}
\end{figure}
In this section, we delve further into the behavior of uncertainties in our approach. To concentrate solely on the recognition model and circumvent uncertainties introduced by the tracker, the results displayed here utilize the ground truth tracking of the target. 
The uncertainty and corresponding final success rate across different difficulty levels are jointly depicted on the left of Figure.~\ref{fig:uncertainty}.
For clarity, the uncertainty used to construct the left sub-figure is the average of single-step uncertainties across all test instances. As we use the ground truth tracking box, the uncertainty generally remains at a low level.
Furthermore, it can be observed that the uncertainty increases with higher recognition challenges, indicating its potential ability to discern challenging recognition queries.

The trends of step-by-step fused uncertainties and success rates are reported on the right side of Figure.~\ref{fig:uncertainty}. The fused uncertainty decreases and recognition improves as more observations are taken, indicating that the proposed agent effectively gathers evidence to support prediction-making. 
Additionally, we include the uncertainty before fusion for reference (represented by the dotted red curve), which is independently predicted based on the current view.


\subsection{Ablation Studies}


\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\linewidth]{figures/results/success_by_step.pdf}
    \caption{Performance between different agents over recognition steps.}
    \label{fig:succ_by_step}
\end{figure}

\begin{table}[t]
\centering
\scriptsize
\caption{Ablation studies about policies, the evidential fusion, and the uncertainty-aware reward.}
    \label{tab:ablation}
    \begin{tabular}{c|c|c|c|cc}
    \hline
    \multirow{2}{*}{\textbf{Method}} & \textbf{Easy} & \textbf{Moderate} & \textbf{Hard} & \multicolumn{2}{c}{\textbf{All}} \\ \cline{2-6} 
     & \textit{\textbf{top-1}} & \textit{\textbf{top-1}} & \textit{\textbf{top-1}} & \multicolumn{1}{c|}{\textit{\textbf{top-1}}} & \multicolumn{1}{c}{\textit{\textbf{top-3}}} \\ \hline\hline
    Ours & {\bf{65.1}} & {\bf{56.0}} & {\bf{51.6}} & \multicolumn{1}{c|}{{\bf{59.2}}} & {\bf{79.1}} \\ \hline
    w/ {\textit{Random}} & 62.1 & 49.6 & 38.2 & \multicolumn{1}{c|}{53.1} & 76.4 \\ \hline
    w/ {\textit{Fixation}} & 63.7 & 55.2 & 51.0 & \multicolumn{1}{c|}{58.4} & 77.9 \\ \hline\hline
    w/ {\textit{Mean evidence}} & 64.6 & 55.3 & 49.4 & \multicolumn{1}{c|}{58.5} & 78.6 \\ \hline
    w/o $u^t$-aware reward & 64.8 & 55.4 & 43.0 & \multicolumn{1}{c|}{57.2} & 78.3 \\ \hline
    \end{tabular}
% \vspace{-5pt}
\end{table}

% \begin{minipage}{0.4\textwidth}
%     \centering
%     \includegraphics[width=1\linewidth]{figures/results/success_by_step.pdf}
%     \captionof{figure}{Performance between different agents over recognition steps.}
%     \label{fig:succ_by_step}
% \end{minipage}
% \vspace{2mm}
% \begin{minipage}{0.58\textwidth}
%     \centering
%     \scriptsize
%     \captionof{table}{Ablation studies about policies, the evidential fusion, and the uncertainty-aware reward.}
%     \begin{tabular}{c|c|c|c|cc}
%     \hline
%     \multirow{2}{*}{\textbf{Method}} & \textbf{Easy} & \textbf{Moderate} & \textbf{Hard} & \multicolumn{2}{c}{\textbf{All}} \\ \cline{2-6} 
%      & \textit{\textbf{top-1}} & \textit{\textbf{top-1}} & \textit{\textbf{top-1}} & \multicolumn{1}{c|}{\textit{\textbf{top-1}}} & \multicolumn{1}{c}{\textit{\textbf{top-3}}} \\ \hline\hline
%     Ours & {\bf{65.1}} & {\bf{56.0}} & {\bf{51.6}} & \multicolumn{1}{c|}{{\bf{59.2}}} & {\bf{79.1}} \\ \hline
%     w/ {\textit{Random}} & 62.1 & 49.6 & 38.2 & \multicolumn{1}{c|}{53.1} & 76.4 \\ \hline
%     w/ {\textit{Fixation}} & 63.7 & 55.2 & 51.0 & \multicolumn{1}{c|}{58.4} & 77.9 \\ \hline\hline
%     w/ {\textit{Mean evidence}} & 64.6 & 55.3 & 49.4 & \multicolumn{1}{c|}{58.5} & 78.6 \\ \hline
%     w/o $u^t$-aware reward & 64.8 & 55.4 & 43.0 & \multicolumn{1}{c|}{57.2} & 78.3 \\ \hline
%     \end{tabular}
%     \label{tab:ablation}
% \vspace{2mm}
% \end{minipage}
% 1. Fixation does not bring much information as the agent just turn left and right
% 2. We use gt tracking results to avoid the influence of visual tracking.
In this study, we explore the impact of various factors such as different policies, evidence fusion methods, and training rewards on our performance. 
To eliminate any unrelated interference, we employ ground truth tracking results and the same visual recognition model for all methods discussed in this section.
Initially, we juxtapose heuristic policies, that is, {\textit{Random}} and {\textit{Fixation}}, against our policy which has been learned with uncertainty-aware rewards. 
The proposed method demonstrates superior performance over both policies. This is primarily because the {\textit{Random}} policy is prone to losing sight of the target easily, while the {\textit{Fixation}} policy does not contribute significant information once the target appears at the center of the view.

We then examine the proposed evidence fusion method, comparing it with the {\textit{Mean evidence}}, which averages estimated beliefs over all frames without considering uncertainty.
A noticeable drop in performance in {\textit{Mean evidence}} can be interpreted as an advantage of proposed evidence fusion.
Furthermore, we assess the performance of our model when uncertainty-aware rewards are not utilized during policy learning. 
In this scenario, a binary reward is provided to the policy based on the current prediction. The comparison emphasizes the efficacy of the proposed reward during training, especially for "hard" testing instances that contain high ambiguities. 
Essentially, this also validates the importance of managing challenges inherent in open environments.

\subsection{Limitations and Future Works}
% Limitations: 
%   a. does not fully measure the uncertainty in the tracking system.
%   b. the action space. how to evaluate when the agent could stop.
In our experiments, recognition performance is evaluated with a predetermined number of total steps, yet an ideal agent would be able to determine when to cease taking more movements. 
Accordingly, as both recognition accuracy and the number of visual observations vary, an effective evaluation metric is further required.
We also find the performance of tracking brings non-negligible impacts to the performance of our proposed method. The uncertainty introduced by the visual tracker needs to be accounted for during active recognition. We leave the investigation for our future work.

==> sec/7_conclusion.tex <==
\section{Conclusions}
\label{sec:conclusion}
% 1. Contributions
%   a. Evidential active recognition to handle open.
%   b. A dataset.
%   d. Experiments
In this paper, we examine the challenges faced when deploying active recognition agents in open-world environments, specifically, how to avoid negative impacts from unexpected inputs in class prediction and policy learning.
These challenges are inherent in active recognition due to the unpredictable and open nature of the environments being explored. 
To address this, we propose to model the recognition as a sequential evidence-collecting process, leading to an uncertainty-aware agent.
Observations from unknown classes or highly ambiguous views can be rejected, fostering more stable and effective policy learning.
A reduced hypothesis space is introduced for knowledge fusion, generating the final opinion in accordance with evidence combination theory. 
A new dataset annotated with recognition difficulty levels is introduced to evaluate different agents.
Experiments on the dataset, along with the uncertainty analysis and ablation studies, confirm the effectiveness of our proposed method.
